Time Efficiency in Optimization with a Bayesian-Evolutionary Algorithm

Not all generate-and-test search algorithms are created equal. Bayesian Optimization (BO) invests a lot of computation time to generate the candidate solution that best balances the predicted value and the uncertainty given all previous data, taking increasingly more time as the number of evaluations performed grows. Evolutionary Algorithms (EA) on the other hand rely on search heuristics that typically do not depend on all previous data and can be done in constant time. Both the BO and EA community typically assess their performance as a function of the number of evaluations. However, this is unfair once we start to compare the efficiency of these classes of algorithms, as the overhead times to generate candidate solutions are significantly different. We suggest to measure the efficiency of generate-and-test search algorithms as the expected gain in the objective value per unit of computation time spent. We observe that the preference of an algorithm to be used can change after a number of function evaluations. We therefore propose a new algorithm, a combination of Bayesian optimization and an Evolutionary Algorithm, BEA for short, that starts with BO, then transfers knowledge to an EA, and subsequently runs the EA. We compare the BEA with BO and the EA. The results show that BEA outperforms both BO and the EA in terms of time efficiency, and ultimately leads to better performance on well-known benchmark objective functions with many local optima. Moreover, we test the three algorithms on nine test cases of robot learning problems and here again we find that BEA outperforms the other algorithms.

==> discussion.tex <==
% Summarize your key findings
% In optimization problem, algorithms take different overhead time and tasks have different evaluation times. Therefore, the performance of algorithms should be evaluated fairly from time efficiency by fitness over computation time. However, algorithms are typically evaluated from data efficiency by fitness over evaluations. BO and EA perform high data efficiency and time efficiency respectively. We therefore propose the algorithm BEA by combining BO and EA to obtain both high data efficiency and time efficiency. In this section, we discuss the results on test functions and the application in terms of time efficiency and data efficiency. 
Throughout the paper we claim that a fair comparison of optimization algorithms should reflect not only sample-efficiency, but also time-efficiency. In the experiments we have presented that indeed the sample-efficiency could be very misleading for a optimization method selection. In the following subsections, we provide a concise discussion of the carried-out experiments.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{On Test Functions}
\label{subsec:disc_function}
%
% The results indicate that…
% The study demonstrates a correlation between…
% The analysis confirms…
% The data suggests that…
% The obtained results on three benchmark functions demonstrate that it is indeed important to evaluate the performance of algorithms in terms of time-efficiency rather than data-efficiency alone. 
BO performs high data-efficiency and time-efficiency for a task in the first a few hundred of evaluations, however, it becomes hardly usable for large number of evaluations due to the cubic overhead time problem.
On the other hand, BEA achieves the higher data-efficiency and time-efficiency than BO by switching to the EA from BO for further learning and inheriting the low time-efficiency of EA.
The switch point in BEA is an important parameter that affects its final performance, and its value changes for different tasks
% It differs from tasks with various complexities and evaluation times.
For instance, the Schewefel function has various switch points for the evaluation times, $0.1, 1, 10$ seconds, namely, 190, 250, 280,  respectively (see \autoref{fig:gain/s-bo-ea}).
% For the same evaluations time, 0.1 seconds, the tasks of Griewank, Rastrigin, and Schwefel function with different complexities need different switch points of 280, 240, 190 respectively.
Moreover, for the same evaluation time, but different test function, the switch points are different (280, 240, 190 for Griewank, Rastrigin and Schwefel, respectively).
% Therefore, we propose the method to test the switch point for different tasks and give the recommended range of switch point value for the types of tasks as test function and application in evolutionary robotics. 
Therefore, it is important to determine the switch point. The method proposed in this paper, which is based on the gain per second, seems to be a reasonable solution.

\par The second stage of BEA aims to transfer the previous solutions with high fitness and high diversity to the EA of BEA. 
Therefore, it is reasonable that the solution S4 by clustering the top $50\%$ outperforms other solutions.
The EA in BEA further obtains rapid learning based on the transferred solutions from BO as shown in the curves after purple lines in \autoref{fig:time-efficiency} and \autoref{fig:applications}.
BO search the space to build the surrogate model using all previous data.
Therefore, it takes many iterations to update the surrogate model and find a better solution.
More and more iterations are required to find a better solution over evaluations.



% Give your interpretations, Interpretations: what do the results mean?

% Discuss the implications,Implications: why do the results matter?

% Acknowledge the limitations,Limitations: what can’t the results tell us?

% State your recommendations,Recommendations: what practical actions or scientific studies should follow?
% What to leave out of the discussion

\todo[inline]{here}  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{On Real-world Applications}
\label{subsec:disc_applications}
%
to do here
%
% \begin{table*}[!ht]
%     \centering
%     \small
%     \setlength\tabcolsep{6pt} % default value: 6pt
%     \begin{tabular}{l|ll|lll|lll|lll}
%     \toprule
%     \multicolumn{3}{c|}{tasks} & \multicolumn{3}{c|}{DL} 
%                   & \multicolumn{3}{c|}{GL} 
%                   & \multicolumn{3}{c}{Rotating} \\
%     \multicolumn{3}{c|}{robots}  &  \multicolumn{1}{c}{S9} & \multicolumn{1}{c}{G7} & \multicolumn{1}{c}{BA} & \multicolumn{1}{|c}{S9} & \multicolumn{1}{c}{G7} & \multicolumn{1}{c}{BA} & \multicolumn{1}{|c}{S9} & \multicolumn{1}{c}{G7} & \multicolumn{1}{c}{BA} \\ \midrule
%     \multirow{2}{*}{fitness} & \multirow{4}{*}{BEA$\rightarrow$} 
%                              & BO   & +22.9\% & +35.6\% & +33.6\% & +12.2\% & +16.7\%& +17.4\% & +11.5\% & +12.8\% & +17.3\%\\
%                           & & EA  & +45.9\% & +69.7\% & +58.7\% & +33.5\% & +68.3\% & +41.9\% & +35.4\% & +26.6\% & +44.7\% \\ \cline{1-1} \cline{4-12}
%     \multirow{2}{*}{time}  & & BO   & 31.0\% & 33.8\% & 32.4\% & 22.8\% & 18.5\% & 22.0\% & 12.8\% & 11.1\% & 13.8\%\\
%                           & & EA  & 112.2\% & 119.6\% & 110.4\% & 114.0\% & 111.3\% & 121.0\% & 111.7\% & 122.7\% & 121.2\%\\ \bottomrule
%     \end{tabular}
%     \caption{The resulting increment in terms of fitness that BEA compared to BO and EA, and percentage of BEA over BO and EA in terms of computation time. We use the abbreviations, DL: directed locomotion; GL: gait learning; S9: the robot ``spider9''; G7: the robot ``gecko7''; BA: the robot ``babyA''.}
%     \label{tab:comparison}
% \end{table*}
% %

% \begin{table*}[!ht]
%     \centering
%     \small
%     \setlength\tabcolsep{6pt} % default value: 6pt
%     \begin{tabular}{ll|lll|lll|lll}
%     \toprule
%     \multicolumn{2}{c|}{tasks} & \multicolumn{3}{c|}{DL} 
%                   & \multicolumn{3}{c|}{GL} 
%                   & \multicolumn{3}{c}{Rotating} \\
%     \multicolumn{2}{c|}{robots}  &  \multicolumn{1}{c}{S9} & \multicolumn{1}{c}{G7} & \multicolumn{1}{c}{BA} & \multicolumn{1}{|c}{S9} & \multicolumn{1}{c}{G7} & \multicolumn{1}{c}{BA} & \multicolumn{1}{|c}{S9} & \multicolumn{1}{c}{G7} & \multicolumn{1}{c}{BA} \\ \midrule
%     \multirow{2}{*}{BO}    & fitness   & +18.7\% & +25.1\% & +18.8\% & +18.9\% & +44.2\%& +20.9\% & +21.5\% & +12.2\% & +23.4\%\\
%                           & time   & +261.6\% & +253.6\% & +241.2\% & +399.2\% & +502.0\% & +449.4\% & +775.7\% & +1000.7\% & +780.8\%\\ \midrule
%     \multirow{2}{*}{BEA}  & fitness   & +45.9\% & +69.6\% & +58.7\% & +33.5\% & +68.3\% & +41.9\% & +35.4\% & +26.6\% & +44.7\% \\
%                           & time   & +12.2\% & +19.6\% & +10.4\% & +14.0\% & +11.3\% & +21.0\% & +11.7\% & +22.7\% & +21.2\%\\
%     \bottomrule
%     \end{tabular}
%     \caption{The resulting increment in terms of fitness and computation time that BO and BEA compared to EA. We use the abbreviations, DL: directed locomotion; GL: gait learning; S9: the robot ``spider9''; G7: the robot ``gecko7''; BA: the robot ``babyA''.}
%     \label{tab:comparison}
% \end{table*}
% %

